Bias Reduction for Sum Estimation

In classical statistics and distribution testing, it is often assumed that elements can be sampled from some distribution $P$, and that when an element $x$ is sampled, the probability $P$ of sampling $x$ is also known. Recent work in distribution testing has shown that many algorithms are robust in the sense that they still produce correct output if the elements are drawn from any distribution $Q$ that is sufficiently close to $P$. This phenomenon raises interesting questions: under what conditions is a "noisy" distribution $Q$ sufficient, and what is the algorithmic cost of coping with this noise? We investigate these questions for the problem of estimating the sum of a multiset of $N$ real values $x_1, \ldots, x_N$. This problem is well-studied in the statistical literature in the case $P = Q$, where the Hansen-Hurwitz estimator is frequently used. We assume that for some known distribution $P$, values are sampled from a distribution $Q$ that is pointwise close to $P$. For every positive integer $k$ we define an estimator $\zeta_k$ for $\mu = \sum_i x_i$ whose bias is proportional to $\gamma^k$ (where our $\zeta_1$ reduces to the classical Hansen-Hurwitz estimator). As a special case, we show that if $Q$ is pointwise $\gamma$-close to uniform and all $x_i \in \{0, 1\}$, for any $\epsilon > 0$, we can estimate $\mu$ to within additive error $\epsilon N$ using $m = \Theta({N^{1-\frac{1}{k}} / \epsilon^{2/k}})$ samples, where $k = \left\lceil (\log \epsilon)/(\log \gamma)\right\rceil$. We show that this sample complexity is essentially optimal. Our bounds show that the sample complexity need not vary uniformly with the desired error parameter $\epsilon$: for some values of $\epsilon$, perturbations in its value have no asymptotic effect on the sample complexity, while for other values, any decrease in its value results in an asymptotically larger sample complexity.

==> preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}


==> sum-estimation-old.tex <==
\section{Old Sum Estimation}
\label{sec:sum-estimation-old}

\begin{algorithm}
$s = \ctodo V \frac{\binom{k}{r}^2 k}{a^2}$\\
$t = \ctodo \sqrt[k]{s n^{k-1}}$\\
$\Xx \leftarrow $ take $t$ samples from $\Ss$\\
$\Xx_r \leftarrow$ $r$-collisions in $\Xx$\\
$A \leftarrow \sum_{x \in \Xx_r} x/\hat{p}(x)^{r}$

\Return{$A/\binom{t}{r}$}
\caption{$SubEstimator(r, k, V)$}
\end{algorithm}

\begin{algorithm}
\Return{$\sum_{i=1}^k(-1)^{i+1} \binom{k}{i} SubEstimator(i, k , V)$}
\caption{$EstimateSum(k, V)$}
\end{algorithm}

\begin{lemma}
Assume $k \leq \frac{1}{2}\log(n a/V)$. Let $Y$ be the estimate returned by $SubEstimator(r)$. Then $E(Y) = \sum_{i=1}^n p(x_i)^r x_i/\hat{p}(x_i)^r$ and $Var(Y) \leq \ctodo a^2/(\binom{k}{r}^2 k)$. The sample complexity of $SubEstimator(r)$ is $O\left(\sqrt[r]{V \binom{k}{r}^2 k n^{r-1} / a^2}\right)$.
\end{lemma}
\begin{proof}
%By linearity of expectation, it holds that $E(ReduceVariance(s_i)) = x_i$. It holds $Var(ReduceVariance(s_i)) = Var(X)/\lceil B_{EV} /V\rceil \leq V$.

We now argue expctation. Consider $S \in \binom{\Ss}{r}$ and let $X_{S, i}$ be the indicator for $a_1 = \cdots = a_r = s_i$. It then holds $E(X_{S,i} s_i/\hat{p}(s_i)) = p_i^k s_i / \hat{p}(s_i)$ as $P(X_{S,i} = 1) = p_i^k$. We now have
\begin{align}
E(A) =& E(\sum_{x \in \Xx_r} x/\hat{p}(x)^r) = E(\sum_{\substack{S \in \binom{\Ss}{r},\\i \in [n]}} X_{S,i} x/\hat{p}(x)^r) = \binom{t}{r}\sum_{i=1}^n p(x_i)^r x_i/\hat{p}(x_i)^r
\end{align}
The algorithm returns $A$ scaled by $1/\binom{t}{r}$. It thus holds $SubEstimator(r) = \sum_{i=1}^n p(x_i)^r x_i/\hat{p}(x_i)^r$.

\jakub{The rest of the proof is not finished. Please ignore it, I'll take care of it.}

We now argue the variance. Since $k \leq \frac{1}{2} \log(n a/V)$, it holds $s \leq n$. Let us number arbitrarily the samples in $\Xx$ and call them $X_1, \cdots, X_t$. Let $Y^i$ be the output that the algorithm would give if $X_i$ were reduced from $\Xx$. Let $T_i$ be the number of times $s_i$ is sampled. Let $j$ be such that $X=s_j$. It holds
\[
Var(Y) \leq \sum_{i=1}^n \inf_{Z_i} E((Y - Z_i)^2) \leq \sum_{i=1}^n E((Y - Y_i)^2) \leq \sum_{i=1}^n E( T_i^{2k})
\]
where the infimum is over $Z_i$ being an $(X_1, \cdots, X_{i-1},X_{i+1},\cdots,X_t)$-measurable random variable, and the explanation of each (in)equality follows. The first inequality is (a variant of) the Efron-Stein equality. The first equality is because $Z$ is a symmetric function of $X_1, \cdots, X_t$ and these random variables are independent. The number of times $s_i$ is sampled is thus distributed as $Bin(t,p_i)$. As such, it holds,
\jakub{This computation is wrong, but the result should be right}
\[
E(T_i^{2k}) = \int_0^\infty P(T_i^{2k} \geq x) dx = \int_0^\infty  P(T_i \geq x^{1/(2k)}) dx = 2k \int_0^\infty x^{2k-1} P(T_i \geq x) dx \leq \mu^{2k} + 2k \int_{\mu}^\infty x^{2k-1} e^{- x} \leq O(k! \mu^{2k}) + O(\mu)
\]
\end{proof}

\begin{lemma}
For all $j$ satisfying $0 \leq j \leq k$
\begin{equation}
\sum_{h=1}^k (-1)^{h+1}\binom{k}{h} \binom{h}{j} =
\begin{cases}
	1 & \mbox{if } j = 0 \\
	(-1)^{k+1} & \mbox{if } j = k \\
	0 & \mbox{otherwise}.
\end{cases}
\label{eqn:binom-identity}
\end{equation}
\end{lemma}
\begin{proof}
We first recall two identities:
\begin{align}
    \sum_{h = 0}^k (-1)^h \binom{k}{h} &= 0, \qquad\text{and} \label{eqn:zero}\\
    \binom{k}{h} \binom{h}{j} &= \binom{k}{j} \binom{k-j}{h-j}. \label{eqn:reduce}
\end{align}
Equation~(\ref{eqn:zero}) follows from the binomial theorem (as the left hand side is equal to $(1 - 1)^k = 0$), while Equation~(\ref{eqn:reduce}) can be derived from the expression $\binom{k}{h} = \frac{k!}{h! (k-h)!}$. The case of the lemma $j = 0$ follows from~(\ref{eqn:zero}). In the case $j = k$, only the term $h = j = k$ is non-zero, in which case the sum evaluates to $(-1)^{h+1}$. Finally, consider the general case $0 < j < k$. We compute
\begin{align}
    \sum_{h = 1}^{k} (-1)^{h+1} \binom{k}{h}\binom{h}{j} &= 
    \sum_{h = j}^k (-1)^{h+1} \binom{k}{h}\binom{h}{j}\\
    &= \sum_{h = j}^k (-1)^{h+1} \binom{k}{j}\binom{k-j}{h-j}\\
    &= - \binom{k}{j} \sum_{h = j}^k (-1)^{h} \binom{k-j}{h-j}\\
    &= (-1)^{j+1} \binom{k}{j} \sum_{h' = 0}^{k-j} (-1)^{h'} \binom{k-j}{h'}\\
    &= 0.
\end{align}
The first equality holds because $\binom{h}{j} = 0$ for $h < j$. The second equality holds by~(\ref{eqn:reduce}), and the final equality by~(\ref{eqn:zero}). This gives the desired result.
\end{proof}

\begin{theorem}
Let $\Ss$ be a multiset of $n$ numbers. Suppose we have access to $(1+\gamma)$-pointwise close to some distribution $Q$ on $\Ss$. Then \Cref{alg:?} returns $\hat{\mu}$ such that $E(\hat{\mu}) = (1\pm\epsilon) \sum \Ss$. If $Var(Q) \leq V$, then $P(|\hat{\mu} - \sum \Ss)| \leq a) \geq 2/3$. Let $k = \lceil \log(\epsilon)/\log(\gamma) \rceil$. If $k \leq O(\sqrt{\log (n a^2/V}))$, it has sample complexity 
\[
O\left(\sqrt[k]{V n^{k-1} / a^2}\right)
\]
Otherwise, the sample complexity is 
\[
O\left(k^2 \sqrt[k]{V n^{k-1} / a^2}\right)
\]
\end{theorem}
\begin{proof}
We can simplify
\begin{align}
E(SubEstimator(r)) = \sum_{i=1}^n p(x_i)^r x_i/\hat{p}(x_i)^r = \sum_{i=1}^n (1+\epsilon_i)^r x_i = \sum_{i=1}^n x_i \sum_{j=0}^r \binom{r}{j} \epsilon_i^j
\end{align}
Using this, we have that
\begin{align}
E(\hat{\mu}) &= \sum_{h=1}^k (-1)^{h+1} \binom{k}{h} \sum_{i=1}^n x_i \sum_{j=0}^r \binom{k}{j} \epsilon_i^j \\
&= \sum_{i=1}^n x_i \sum_{h=1}^k \sum_{j=0}^h (-1)^{h+1} \binom{k}{h} \binom{h}{j} \epsilon_i^j \\
&= \sum_{j=1}^n x_i \sum_{j=0}^k \sum_{h=1}^k (-1)^{h+1}\binom{k}{h} \binom{h}{j} \epsilon_i^j \\
&= \sum_{j=1}^n x_i \sum_{j=0^k} \epsilon_i^j \sum_{h=1}^k (-1)^{h+1}\binom{h}{j} \binom{k}{h} \\
&= \sum_{j=1}^n x_i (1+ (-1)^{k}\epsilon_i^k)
\end{align}
where the last equality holds by \Cref{lem:?}

The variance of $(-1)^{i+1} \binom{k}{i} SubEstimator(i)$ is $((-1)^{i+1} \binom{k}{i})^2 \cdot (\ctodo a^2 /(\binom{k}{i}^2 k) = a^2/k$. It then holds
\[
\sum_{i=1}^{k} Var((-1)^{i+1} \binom{k}{i} SubEstimator(i)) \leq \ctodo a^2
\]
By the Chebyshev inequality, we then have
\[
P(|\hat{\mu} - E(\hat{\mu})| \leq a) \frac{\ctodo a^2}{a^2} \geq 2/3
\]


The asymptotic sample complexity is
\begin{align}
\sum_{i=1}^k \sqrt[r]{V \binom{k}{r}^2 k n^{r-1} / a^2}  = \sum_{i=1}^k \sqrt[r]{V \binom{k}{r}^2 k n^{r-1} / a^2} + 
\end{align}
We now bound this. We define
\begin{align}
C(r) = \sqrt[r]{V \binom{k}{r}^2 k n^{r-1} / a^2} \leq \sqrt[r]{V (\frac{e k}{r})^{2r} k n^{r-1} / a^2} = (\frac{e k}{r})^2 \sqrt[r]{V k n^{r-1} / a^2}
%\sum_{r=1}^{k/2} \sqrt[r]{V k^{r+1} n^{r-1} / a^2} + \sum_{r=k/2+1}^k \sqrt[r]{V k^{k-r+1} n^{r-1} / a^2} 
\end{align}
We first consider the simpler case of $k \geq \sqrt{\log na^2/V}$ (the bound in fact holds for any $k$. It holds
\[
\sum_{r=2}^k C(r) \leq (e k)^2 \sqrt[k]{V k n^{k-1}/a^2} \sum_{r=2}^k \frac{1}{r^2} = O(k^2 \sqrt[k]{V k n^{k-1}/a^2})
\]


We now consider the case $k \leq O(\sqrt{\log na^2/V})$. Consider $C(r)/C(r+1)$. We show that this is bounded away from $1$. This implies that $C(r)$ increases exponentially, implying that the sum $\sum_{r=2}^k C(r)$ is dominated by the last summand $C(k)$. It holds
\begin{align}
C(r)/C(r-1) = \left( \frac{n a^2}{V k}\right)^{\frac{1}{r(r-1)}} \frac{r^2}{(r-1)^2} \geq \left( \frac{n a^2}{V k}\right)^{\frac{1}{r(r-1)}}
\end{align}
Taking logarithms of both sides, we get the first inequality of
\[
\log(C(r)/C(r-1)) \geq \frac{\log(na^2/Vk)}{r(r-1)} \geq \frac{\log(na^2/V)}{4 r^2}
\]
where the second inequality holds because we may assume $k \leq \sqrt{n}$. This is uniformly bounded from $0$. $C(r)/C(r-1)$ is thus uniformly bounded from $1$.
\end{proof}

